Personalized Rollout Allocation for Federated LQR Policy Optimization under Heterogeneous Process Noise

We study federated model-free learning of a common linear quadratic regulator (LQR) gain under a limited uplink communication budget, with clients that share dynamics and costs but experience different process-noise levels. Conventionally, clients transmit gradient matrices whose dimension equals the number of controller parameters. Exploiting the structure of two-point zeroth-order estimates, we consider an implementation in which clients transmit only one scalar cost-difference coefficient per rollout pair, while the server regenerates the associated perturbation directions from shared seeds. Communication thus scales with the number of rollout pairs rather than the controller dimension, turning the uplink budget into a rollout budget. Because noise heterogeneity produces gradient estimates of widely differing variance and every client carries equal weight in the fleet objective, uniform rollout allocation allows noisy clients to dominate the aggregated update and increases the probability of destabilizing updates. We propose a rollout-allocation scheme that assigns rollout pairs in proportion to the standard deviation of each client's estimates and show that it minimizes the variance of the aggregated update. The scheme is implemented exactly through a greedy integer allocation rule whose weights are estimated from the communicated scalars. We further prove that a single allocation factor quantifies its improvement over uniform allocation in a one-round instability bound, the certified step size, and the error floor of a joint stability and convergence guarantee. Simulations show that, under the same communication budget, personalized allocation reduces the one-step instability rate from $37\%$ to $0.3\%$.

==> appraoch.tex <==
\section*{Adaptive Rollout Allocation for Communication-Efficient Model-Free LQR}

The main observation is that, using shared random seeds, the zeroth-order
policy-gradient estimator can be reconstructed at the server from scalar
rollout evaluations. Hence, instead of transmitting a $D$-dimensional policy
gradient, agent $i$ communicates only $m_i$ scalar measurements, where $m_i$
is the number of random perturbation directions assigned to that agent.

We further consider heterogeneous resource constraints. Let $\bar m_i$ denote
the maximum number of directions that agent $i$ can evaluate in one round,
e.g., due to its battery or rollout limitation, and let $B$ denote the total
uplink communication budget at the server. If each scalar requires $b$ bits,
the number of directions is selected by solving
\begin{equation}
\boxed{
\begin{aligned}
\min_{\{m_i\}}
\quad &
\sum_{i=1}^{M}\frac{V_i}{m_i}
\\
\mathrm{s.t.}\quad &
b\sum_{i=1}^{M}m_i\leq B,
\\
&
m_{\min}\leq m_i\leq \bar m_i,
\qquad i=1,\ldots,M ,
\end{aligned}}
\label{eq:rollout_allocation}
\end{equation}
where
\begin{equation}
V_i
\approx
(D-1)\|\nabla J_i(K)\|_F^2
\end{equation}
characterizes the contribution of agent $i$ to the zeroth-order gradient
estimation variance. Since the local gradient is unavailable in the model-free
setting, $V_i$ can be estimated from a small number of pilot directional
evaluations.

Ignoring the integer constraint, the KKT conditions give
\begin{equation}
\boxed{
m_i^\star
=
\left[
\sqrt{\frac{V_i}{\lambda b}}
\right]_{m_{\min}}^{\bar m_i},
}
\end{equation}
where $\lambda$ is selected such that the total communication constraint is
satisfied. Thus, agents with larger gradient/estimation importance receive
more rollout directions, subject to their individual resource limits.

\paragraph{Numerical observation.}
We evaluated the allocation under the same communication budget and policy
dimension $D=144$, while varying only the heterogeneity among the agents.
The results show that the advantage of optimized rollout allocation increases
with the heterogeneity of the local gradient norms:
\begin{center}
\begin{tabular}{c|c|c}
\hline
Heterogeneity & Gradient-norm spread &
MSE reduction of $m_i^\star$ vs. equal
\\
\hline
Low    & $\approx 1.45\times$ & $\approx 2.1\%$ \\
Medium & $\approx 5.5\times$  & $\approx 28.8\%$ \\
High   & $\approx 64.7\times$ & $\approx 65.6\%$ \\
\hline
\end{tabular}
\end{center}

For low heterogeneity, $V_i$ is nearly identical across agents and the optimal
allocation naturally approaches equal allocation. As heterogeneity increases,
the optimized allocation becomes increasingly nonuniform and concentrates the
limited communication/rollout budget on the agents that contribute most to
the global gradient-estimation error. In the high-heterogeneity experiment,
the practical pilot-based allocation also resulted in a substantially smaller
LQR optimality gap than equal or random allocation.

==> longer_intro.tex <==
\section{Introduction}\label{sec:intro}


Networked autonomous systems create opportunities to learn control
policies from trajectory rollouts distributed across fleets of agents.
When similar agents share a common control objective, the rollouts
collected by each system carry complementary information about the same
policy. Aggregating this information informs each policy update with
more rollouts than any single agent could generate, which improves
sample efficiency and reduces the exploration burden on individual
agents. Federated learning provides a natural architecture for this
setting: agents, referred to as clients, generate trajectory rollouts
locally, and a coordinating server aggregates the information extracted
from them to update a common controller. This separation between
distributed data collection and server-assisted policy learning (e.g.,
on a cloud server) is well suited to physical systems, where data are
acquired through interaction and rollouts can be executed in parallel. The benefit of cooperation,
however, is limited by communication, energy, and per-round latency.
Clients typically share a bandwidth-limited wireless uplink, and each
learning round must be completed within a deadline so that policy
updates remain timely while the systems operate; the channel can
therefore deliver only a limited number of transmissions to the server
in each round. Clients also operate on energy-constrained platforms, for
which every rollout and every transmission consumes battery capacity
that is shared with the primary task. Together, these constraints cap
the total uplink traffic that the fleet can generate per round, so
uplink communication is a scarce~resource that must be allocated across
clients rather than spent uniformly.

This paper considers federated learning of a common linear quadratic
regulator (LQR) gain from model-free trajectory rollouts. In each round,
the server broadcasts the current controller, each client executes
trajectory rollouts with perturbed versions of it, and the server
aggregates the results to update the shared gain. The number of rollouts
governs the quality of learning: the variance of the gradient estimate
decreases in inverse proportion to the number of rollouts, and a more
accurate estimate permits larger and safer policy updates. Although all
clients share the same dynamics and cost, their rollouts are not equally
informative: differences in operating conditions and process-noise
levels produce gradient estimates of substantially different variance.
An effective federated scheme must therefore determine not only how
information is aggregated but also from which clients rollouts should be
solicited when communication is limited.

We consider policy optimization with two-point zeroth-order gradient
estimates, each obtained from a pair of trajectory rollouts at two
symmetrically perturbed gains. Conventionally, each client averages its
local estimates and transmits a gradient matrix whose dimension
$D=n_un_x$ equals the number of controller parameters. Each two-point
estimate, however, is the product of a scalar cost-difference
coefficient and a random perturbation direction. When the directions are
generated from seeds shared with the server, the server reproduces them
and reconstructs the same gradient estimate, so clients need to transmit
only the scalar coefficients. Since each coefficient is tied to its own
direction, the coefficients cannot be aggregated before transmission:
every rollout pair incurs one transmitted scalar. Uplink cost thus
scales with the number of rollouts rather than with $D$, and is lower
than that of matrix transmission whenever a client executes fewer than
$D$ rollout pairs per round. A communication budget is then equivalent
to a rollout budget, and the central design question becomes: given a
fixed number of transmitted scalars per round, from which clients, and
in what numbers, should rollouts be solicited?

Answering this question requires a measure of client effectiveness. We
quantify the effectiveness of a client by the reduction in the variance
of the aggregated gradient estimate that one additional rollout pair
from that client achieves. Because every client carries equal weight in
the fleet objective, this reduction depends on the variance of the
client's coefficients and on the number of rollouts it has already been
assigned: it is large for a client whose estimates are uncertain and
diminishes as more rollouts are assigned to it. Effectiveness therefore
differs from data quality per rollout. A client subject to large process
disturbances returns less reliable coefficients, yet, since its
contribution to the aggregate cannot be discounted, additional rollouts
from it remove more uncertainty than additional rollouts from a
low-noise client. The variance that defines this measure can be
estimated by the server from the coefficients it already receives, at
no additional communication cost.

Uniform allocation ignores this measure and assigns the same number of
rollouts to every client. With few rollouts, high-noise clients then
dominate the aggregated update. In standard stochastic optimization,
such variance primarily slows convergence. In learning-based control, it
can drive the updated gain outside the set of stabilizing controllers or
render the perturbed gains queried for gradient estimation unstable. The
merit of an allocation must therefore be assessed through its effect on
stability guarantees and learning performance, not through variance
alone.

\textit{Related work.} LQR is a canonical benchmark for learning-based
control~\cite{recht2019tour}. Despite the nonconvexity of the set of
stabilizing gains, policy-gradient methods converge
globally~\cite{fazel2018global,bu2019lqr,hu2023toward}, and these
guarantees extend to settings with multiplicative or additive process
noise~\cite{gravell2021learning,hambly2021policy,mohammadi2022convergence,song2025stochastic}.
Model-free methods avoid system identification~\cite{dean2020sample} at
the cost of trajectory rollouts, whose sample complexity and estimation
error are analyzed in~\cite{tu2019gap,malik2019derivative,song2025stochastic};
two-point estimators connect these methods to zeroth-order
optimization~\cite{nesterov2017random,ghadimi2013stochastic,duchi2015optimal,shamir2017optimal}.
Federated formulations of controller learning have addressed
heterogeneous dynamics~\cite{wang2023federated},
meta-learning~\cite{toso2024meta}, variance
reduction~\cite{toso2024oracle}, decentralized
control~\cite{li2022distributed}, and federated reinforcement
learning~\cite{khodadadian2022federated}. In these works, heterogeneity
is modeled through differences in dynamics or tasks; heterogeneity in
the quality of locally collected data has received little attention.

Communication bottlenecks in federated learning have motivated
compressed and quantized update
representations~\cite{mcmahan2017communication,alistarh2017qsgd}. The
scalar-and-seed structure of random-direction estimators has been
exploited to reduce communication in federated zeroth-order
optimization~\cite{fang2022communication,qin2024federated}, and a scalar
communication scheme was recently proposed for federated model-free
LQR~\cite{rostami2026scalar}. These methods solicit the same number of
samples from every client. Nonuniform client sampling and importance
sampling reduce estimator
variance~\cite{chen2022optimal,needell2014stochastic,zhao2015stochastic},
and the resulting square-root rule coincides with Neyman allocation in
stratified sampling~\cite{neyman1934two}; when clients contribute
unequal amounts of local work, their contributions must be normalized to
avoid biasing the objective~\cite{li2020federated,wang2020tackling}.
None of these works, however, relates the allocation to closed-loop
stability or to convergence of learning-based control.

\textit{Contributions.} This paper develops a communication-aware
federated framework for model-free LQR in which clients transmit scalar
coefficients and the server solicits trajectory rollouts according to
the estimated effectiveness of each client. The main contributions are
as follows.
\begin{itemize}
\item We formulate rollout allocation under a fixed scalar
communication budget and derive the variance-optimal allocation, which
assigns rollouts in proportion to the standard deviation of each
client's coefficients. Its exact integer implementation solicits each
rollout pair from the currently most effective client while
guaranteeing minimum client participation, and its weights are
estimated from the received coefficients without additional
communication.
\item We establish a one-round stability certificate that bounds the
probability of a destabilizing update or query. A single allocation
factor $\Gamma_k$ divides this bound and the budget required to certify
stability, and enlarges the certified step size by up to
$\sqrt{\Gamma_k}$.
\item We derive a joint stability and convergence guarantee for the
fleet-averaged LQR objective and show that the same factor reduces its
sampling-error floor.
\end{itemize}
Simulations with ten and twenty clients support the analysis: under the
same budget, personalized allocation reduces the one-step instability
rate from $37\%$ to $0.3\%$ and sustains learning at step sizes for
which uniform allocation fails.


